Towards Explainable Collaborative Filtering with Taste Clusters Learning

Collaborative Filtering (CF) is a widely used and effective technique for recommender systems. In recent decades, there have been significant advancements in latent embedding-based CF methods for improved accuracy, such as matrix factorization, neural collaborative filtering, and LightGCN. However, the explainability of these models has not been fully explored. Adding explainability to recommendation models can not only increase trust in the decisionmaking process, but also have multiple benefits such as providing persuasive explanations for item recommendations, creating explicit profiles for users and items, and assisting item producers in design improvements. In this paper, we propose a neat and effective Explainable Collaborative Filtering (ECF) model that leverages interpretable cluster learning to achieve the two most demanding objectives: (1) Precise - the model should not compromise accuracy in the pursuit of explainability; and (2) Self-explainable - the model's explanations should truly reflect its decision-making process, not generated from post-hoc methods. The core of ECF is mining taste clusters from user-item interactions and item profiles.We map each user and item to a sparse set of taste clusters, and taste clusters are distinguished by a few representative tags. The user-item preference, users/items' cluster affiliations, and the generation of taste clusters are jointly optimized in an end-to-end manner. Additionally, we introduce a forest mechanism to ensure the model's accuracy, explainability, and diversity. To comprehensively evaluate the explainability quality of taste clusters, we design several quantitative metrics, including in-cluster item coverage, tag utilization, silhouette, and informativeness. Our model's effectiveness is demonstrated through extensive experiments on three real-world datasets.

==> 2_methodology_old.tex <==
\section{Methodology}
In this section, we first introduce the definition of taste cluster and the problem formulation. Then we detail the learning paradigm of taste clusters, as well as the end-to-end optimization methods. 
% Besides, the forest mechanism of ECF is demonstrated to enhance the accuracy and diversity. 
Finally, we also describe how to achieve explanation and recommendation with the proposed ECF.

\subsection{Problem Formulation}
% We first introduce the definition and data related to our studied problem, and then formulate our task.

\vspace{3pt}
\noindent
\textbf{User-item Interactions and Tags.} Let $M$ and $N$ denote the number of users and items, respetively. We define the user-item interaction matrix $\Mat{Y}\in \Space{R}^{M\times N}$ from users' implicit feedback, where $y_{ui} = 1$ means that there is an interaction between user $u$ and item $i$, otherwise $y_{ui} = 0$. Besides, we also assume that there is a set of tags $\Set{T}= \{t\}$ for items, and each item $i$ can be described by $\Set{T}_i = \{t_{i_1}, t_{i_2},...,t_{i_k}\}$, where $\Set{T}_i \subset \Set{T}$.


\vspace{3pt}
\noindent
\textbf{Taste Clusters.} Let $Z$ denote the number of taste clusters, and each of them is a collection of items $c = \{i_1, i_2,...,i_c\}$, which can be identified with descriptive tags $\Set{T}_c = \{t_{1}, t_{2},...,t_{c}\}$. We define the user- and item- cluster affiliations as $\Mat{A}\in\Space{R}^{M\times Z}$ and $\Mat{X}\in\Space{R}^{N\times Z}$, where $a_{uc}$ indicates the preference of user $u$ to taste cluster $c$ and $x_{ic}$ denotes the belongings between item $i$ and taste cluster $c$. 

\vspace{3pt}
\noindent
\textbf{Explainable Recommendation with Taste Cluster.} Given the user-item interactions and the tags of items, the task of ECF is to (1) generate high-quality taste clusters with informative tags; (2) learn the affiliations between user/item and taste clusters; and (3) make explainable recommendation with taste clusters, as well as the affiliation relationships.

\subsection{Taste Clusters Learning}\label{sec:taste-cluster-learning}
As we mentioned before, a taste cluster should not only reveal the latent interests of users (\ie collaborative similarity), but also can be explicitly distinguished with common tags shared by items within (\ie tag similarity). This is a non-trival task since directly performing clustering algorithm (\eg K-means) for items or blindly collecting items with same tags would fail to encode both hidden and explicit semantics simultaneously (see Section~\ref{sec:eval-explanation} for comparison). Besides, it is also challenging to generate proper tags for taste clusters since they should be neat yet representative for explanation. Moreover, the affiliations between users/items and taste clusters are supposed to be sparse and informative so that we could easily derive the decision logic of ECF. These unsolved issues motivate us to develop a novel taste clusters learning paradigm to generate high-quality taste clusters for transparent and explainable recommendations.

% To begin with, instead of directly generating clusters by applying various clustering algorithms, we aim to embed taste clusters with learnable vectors and optimize them from the following three different aspects.
% This is because that it is hard to constrain the post-generated clusters with both high hidden (collaborative similarity) and explicit (tag similarity) semantics simultaneously.

\subsubsection{\textbf{Collaborative Similarity in Taste Clusters.}} 
We first consider the affiliations relationship between clusters and items by computing their cosine similarity:
\begin{gather}\label{equ:item-cluster-sim}
    \tilde{x}_{ic} = \cos (\Mat{v}_i, \Mat{h}_c)
\end{gather}
where $\Mat{v} \in \Space{R}^{d}$ and $\Mat{h} \in \Space{R}^{d}$ are the embeddings of items and clusters, and $d$ is the embedding size. To clearly identify the belongings between items and clusters, we only consider the Top-$K$ clusters for each item:
\begin{gather}
    \label{equ:mask-item-cluster-sim}
    m_{ic} = \left\{\begin{array}{cl}
    1 & \text { if } c\in \argtop{K} (\tilde{\Mat{x}}_i) \\
    0 & \text { otherwise }
    \end{array}\right. \\
    \Mat{x}_i = \sigma (\tilde{\Mat{x}}_i ) \odot \Mat{m}_i \label{equ:item-cluster-sparse}
\end{gather}
where $\odot$ denotes Hadamard product, $\sigma(\cdot)$ is the sigmoid function. In the above equations, we first apply the sigmoid function to indicate the relatedness of items and clusters with none-zero probabilities, and make Top-$K$ selection for each item according to the relatedness scores, then use a binary mask to filter other less relevant clusters. However, due to the non-differentiability and discrete nature of $\argtop{K}$ operation, the computation is intractable thus cannot be optimized with gradients. Inspired by the widely-used reparameterized trick~\cite{iclr17gumbel}, we detach $\Mat{m}_i$ from the computation graph while multiplying with $\tilde{\Mat{x}}_i$. Therefore, the whole computation is fully differentiable \wrt $\tilde{\Mat{x}}_i$ and can be smoothly optimized with the model.

Next, we use the same mechanism to obtain the affiliations between users and clusters. Specifically, the user-cluster similarity matrix can be computed as:
\begin{gather}\label{equ:user-cluster-sim}
    \tilde{\Mat{A}} = \Mat{Y} \times \tilde{\Mat{X}}
\end{gather}
where $\Mat{Y}$ is the user-item interaction matrix. Then, we also force each user belongs to only Top-$F$ clusters, resulting in the user-cluster affiliation matrix $\Mat{A}$. Finally, given the user- and item-cluster affiliation matrices, we can now predict how likely the user $j$ would adopt an item $i$ through their common taste clusters:
\begin{gather}\label{equ:sparse-prediction}
    \hat{y}_{ui} = \sum\nolimits_{c}^Z a_{uc} \times x_{ic}
\end{gather}
It is worth mentioning that by mapping users and items to their belonging taste clusters, the prediction process can be naturally explained by the affiliations between users/items with taste clusters, which makes our model self-explainable. We opt for BPR loss~\cite{uai09BPRloss} to optimize the predictions:
\begin{gather}\label{equ:sparse-bpr}
    \Lapl_\text{CS} = \sum\nolimits_{(u, i, j) \in \Set{O}}-\ln \sigma(\hat{y}_{u i}-\hat{y}_{u j})
\end{gather}
where $\Set{O} = \{(u,i,j) | y_{ui} = 1, y_{uj} = 0\}$ denotes the training set of user-item interactions.

\subsubsection{\textbf{Tag Similarity in Taste Clusters}} Although we have successfully mapped users/items to the potential taste clusters, the clusters themselves remain to be hidden and intricate. We argue that a good taste cluster should contains items with similar tags, so that it can be easily abstracted with a few common tags. Therefore, we first calculate the tag distribution of taste clusters as follows:
\begin{gather}\label{equ:tag-distribution}
    \tilde{\Mat{D}} =  \Mat{X} \times \Mat{E}
\end{gather}
where \Mat{E} is the multi-hot matrix where each entry $e_{it}$ denotes whether item $i$ has the tag $t$, and $\tilde{\Mat{D}}$ represents the tag frequency within each taste cluster. Intuitively, we can directly select the most frequent tags as the description of taste clusters. However, this would result in the indistinguishability between different clusters, since some tags are commonly shared by most items and they would dominate the tag distribution across different taste clusters. Take the game genres at Xbox dataset as an example. Most of the games are online and allow for mutiplayers, thus selecting the ``MultiplayerOnline'' tag fails to provide informative description for taste clusters. To tackle this problem, we first reweight each tag according to its frequency of occurrence in items, and then compute the weighted distribution:
\begin{gather}\label{equ:tag-tfidf}
    d_{ct} =  \tilde{d}_{ct} \times \log (\frac{N}{f_t + \epsilon})
\end{gather}
where $N$ is the number of items, $f_t$ is the frequency of tag $t$ across all items, and $\epsilon$ is a small fraction (we set it as $10^{-6}$) to avoid numerical overflow. Thus, above equation considers both tag frequency and items' affiliations for tag informativeness: the more frequent the distinctive tag appears, the more informative it is for interpreting the taste clusters.

Besides, to facilitate the understanding of taste clusters, we argue that the number of tags generated for taste clusters should not be too small or too large. This is because that disproportionate number of tags would be too abstract or too complex to identifying users' true interests, thus makes it difficult to interpret. Thus, we first  normalize their importance scores as:
\begin{gather}\label{equ:tag-softmax}
    \beta_{ct} =  \frac{\exp (\log (d_{ct})/\tau)}{\sum\nolimits_{c_j\in\Set{T}}\exp (\log (d_{ct})/\tau)}
\end{gather}
where $\tau$ is the is a hyperparameter called \textit{temperature}, which control the control the entropy of the tag distribution. For low temperatures, the distribution becomes more sharp, thus only the tag with highest score would stand out. As the temperature increases, the distribution becomes more even and the distinctiveness between tags will decrease (we set $\tau=2$ for all experiments). Then, we consider to maximize the likelihood of the probabilities of Top-$P$ tags so that the taste clusters can be easily identified with those tags:
\begin{gather}\label{equ:tag-likelihood}
    \Lapl_\text{TS} = \sum\nolimits_{c \in \Set{C}} \sum\nolimits_{t\in \argtop{P}(\beta_{c})}-\log \beta_{ct}
\end{gather}
where $\Set{C} = \{c_1,c_2,...c_Z\}$ denotes the set of taste clusters. We fix the number of tags $P=4$ for all experiments, since it achieve a good balance between informativeness and readability.


\subsubsection{\textbf{Independence Modeling of Taste Clusters}} Different taste clusters should contain different items and reveal different user preference, so that the latent interest space could be better preserved. Hence, for better model capacity and diversity, we encourage the embeddings of taste clusters to differ from each others. Here we introduce a module of independence modeling to guide the learning of independent taste clusters. This module can be simply achieved by applying a statistical measure, such as distance correlation~\cite{07pearson}, orthogonality~\cite{ijcai19hifi}, and mutual information~\cite{icml18mutual,www21kgin}. Here we offer three alternative implementations:
\begin{itemize}[leftmargin=*]
    \item \textbf{Distance correlation.} It measures both linear and nonlinear associations of any two variables, whose coefficient is zero if and only if these variables are independent. Minimizing the distance correlation of taste clusters enables us to reduce the dependence of different clusters, which is formulated as:
    \begin{gather}\label{equ:distance-correlation}
    \Lapl_\text{IND} = \sum\nolimits_{c,c^\prime \in \Set{C}, c^\prime\neq \Set{C}} \frac{\dcov(\Mat{h}_c, \Mat{h}_{c^\prime})}{\sqrt{\dvar(\Mat{h}_c) \cdot \dvar(\Mat{h}_{c^\prime})}}
    \end{gather}
    where $\dcov(\cdot)$ denotes the distance covariance of two taste clusters, and $\dvar(\cdot)$ is the distance variance of each taste cluster.
    \item \textbf{Orthogonality.} To exclude redundancy for taste clusters, we can directly force their embeddings to be orthogonal as much as possible, and it can be formulated as follows:
    \begin{gather}\label{equ:orthogonal}
    \Lapl_\text{IND} = ||\Mat{H}\Mat{H}^T \odot  (\Mat{J} - \Mat{I})||_{F}
    \end{gather}
    where $||\cdot||_{F}$ denotes the Frobenius norm, $\Mat{H}\in \Space{R}^{Z\times d}$ is the embedding matrix of taste clusters, and $\Mat{J}, \Mat{I} \in\Space{R}^{Z\times Z}$ are the all-one and identity matrices, respectively. As a result, orthogonality indicates that the inner products between different taste clusters are forced to be zeros.
    \item \textbf{Mutual information.} We minimize the mutual information between the embeddings of any two different taste clusters, so as to quantify their independence:
    \begin{gather}\label{equ:mutual-information}
    \Lapl_\text{IND} = \sum\nolimits_{c \in C} -\log \frac{\exp(s(\Mat{h}_c,\Mat{h}_c)}{{\sum\nolimits_{c^\prime \in C}\exp(s(\Mat{h}_c,\Mat{h}_{c^\prime})}}
    \end{gather}
    where $s(\cdot)$ is the similarity function to measure the associations of any two taste clusters, which is set as cosine function here. We use this constraint for all experiments due to its simplicity.
    
\end{itemize}


\subsection{Optimization of ECF}
\subsubsection{\textbf{Learning with Collaborative Signals}}\label{sec:opt-cf}
We consider to learn taste clusters by putting above objective functions together:
\begin{gather}\label{equ:taste-cluster-loss}
\Lapl_\text{TC} = \Lapl_\text{CS} + \Lapl_\text{TS} + \Lapl_\text{IND}
\end{gather}
Note that we do not need to tune any weighting coefficients for each loss, since each of them define a essential aspect that the taste clusters should accomplish, and our experiments on three datasets also show the robustness of overall loss function. Ideally, we can directly optimize Equation (\ref{equ:taste-cluster-loss}) to learn taste clusters as well as the recommendations. However, since the objective functions of the taste clusters learning are sparse (\eg Top-$K$ operations), directly optimizing with gradient descent optimization methods would suffers from convergence problem. Thus, we aim to add auxiliary supervised signals from traditional embedding-based collaborative filtering methods (\ie MF):
\begin{gather}\label{equ:dense-loss}
\Lapl_\text{CF} = \sum\nolimits_{(u, i, j) \in \Set{O}}-\ln \sigma(\Mat{e}_u^{\top} \Mat{v}_i - \Mat{e}_u^{\top} \Mat{v}_j)
\end{gather}
where $\Mat{e}_u$ denotes the embeddings of user $u$. We choose inner product of embeddings to measure the similarity between users and items for simplicity, but more sophisticated embedding-based models (\eg LightGCN~\cite{sigir20lighGCN}) can also be applied, which will be discussed in Section~\ref{sec:further-study}. By combing the taste clusters loss and collaborative loss, we minimize the following objective function to learn the model parameters:
\begin{gather}\label{equ:ecf-loss}
\Lapl_\text{ECF} = \Lapl_\text{TC} + \lambda \Lapl_\text{CF}
\end{gather}
where $\lambda$ a hyperparameter to control the impact of auxiliary collaborative signals.

\subsubsection{\textbf{Optimization with Activated Taste Clusters}}\label{opt-cluster}
We opt for the standard iterative optimization methods (\ie Adam~\cite{iclr14adam}) to train the model. However, directly leveraging taste clusters as the training data is infeasible since the number of taste clusters is a hyperparameter (usually quiet small) thus it is hard to determine the batch size. A large batch size may be out of proportion with the number of taste clusters, and resulting in poor generalization~\cite{iclr17batch}. Besides, small-batch methods may easily converge to flat minimum. Therefore, we follow conventional recommendation methods and choose user-item interaction pairs as the training data for optimization. To be specific, for each iteration, users and items in a batch would activate their affiliated taste clusters (see Equation (\ref{equ:item-cluster-sparse}) and Equation (\ref{equ:user-cluster-sim})), and those clusters are chosen to be optimized in this batch while others are masked since no collaborative or tag signals have passed on them. We find this approach is quiet robust for training and it is easy to implement.

Besides, it should be noticed that precisely computing the tag distribution needs to traverse all the items in each taste cluster (see Equation (\ref{equ:tag-distribution})), which suffers from huge computational overhead when the size of items is large in real-world scenario. Thus, instead of directly compute the distribution with all items, we utilize items in a batch to approximate the tag distribution, and the experiments show the effectiveness of this alternative approach.

% \subsubsection{\textbf{Gradient Shielding}}
% Since the training process of taste clusters do not evolve users, we refrain the backpropagation from $\Lapl_\text{TC}$ to the user embedding $\Mat{u}$ to ensure the 

\subsection{Forest mechanism}
Due to the hidden nature of users' interest space, it is hard to determine how many taste clusters are needed to model user preference properly. Besides, training with excessive taste clusters would result in poor performance since we use the batch optimization technique to approximate the true affiliation relationships and distributions. Thus, to improve the diversity and accuracy of recommendation, we propose a simple yet effective ensemble method, called forest mechanism, to substantially enhance the expressiveness of taste clusters learning, while also maintain good explanability. Specifically, for each single ECF model, we randomly select $Z$ items as the initial taste clusters, and using different random seeds for model training. Then we train 9 different model to form the final ECF model. We find this simple random mechanism would boost the performance of ECF and also provide a comprehensive explanation for predictions.


\subsection{Personalized Recommendation}
Given the trained ECF model, we could directly generate the taste clusters with their descriptive tags by selecting top-$P$ tags with highest probability, as described in Equation (\ref{equ:tag-softmax}). Besides, the affiliation relationships between users/items with taste clusters can also be derived from $\Mat{X}$ and $\Mat{A}$. Based on that, top-$K$ recommendation and personalized explanation can be performed simultaneously, as described in the following subsections.

\subsubsection{\textbf{Top-K Recommendation}}
We assume that a user's decision about whether to make a purchase/click is based on his/her preference with taste clusters, as well as the item's affiliations with them. Thus the prediction is directly performed with the two affiliation matrices in Equation (\ref{equ:sparse-prediction}). Then we combine all the ranking scores from each ECF model as the final prediction: 
\begin{gather}\label{equ:ecf-prediction}
r_{ui} = \sum\nolimits_{\Set{C}_i\in\Set{G}} \sum\nolimits_{c\in\Set{C}_i}  a_{uc} \times x_{ic}
\end{gather}
where $\Set{G} = \{\Set{C}\}$ denotes the collection of taste clusters generated by individual ECF model. The top-$K$ recommendation list for user $u$ can be constructed by ranking the items based on $r_{ui}$.


\subsubsection{\textbf{Personalized Explanation}}
Traditional factorization models are usually difficult to understand and hard to generate self-explanaible decision logic about why an item is recommended through the hidden factors. However, an important advantage of our ECF is the ability to automatically generate intrinsic running logic by measuring the coherence between items’ taste cluster affiliations. Specifically, when explaining why item $i$ is recommended to user $u$, we first search for their overlapped taste clusters and corresponding tags:
\begin{gather}\label{equ:ecf-explanation}
\Set{F}_{ui} = F(\Mat{a}_u) \cap F(\Mat{x}_i) 
\end{gather}
where $F(\cdot)$ is an index selector to collect corresponding clusters where the affiliation between users/items and taste clusters exists. Then we generate the importance score for user-item pairs by multiply the weight of affiliations $a_{uc}\times x_{ic}$ of the chosen taste clusters $c$, which is the same with the prediction in Equation (\ref{equ:ecf-prediction}). Finally, the explanation results can be clearly described by a simple template method~\cite{sigir14efm} using the importance scores and tags of the taste clusters.

It is worth noting that, the above explanation mechanism is completely consist with the decision process of ECF, while previous works~\cite{sigir14efm,ijcai20amcf} typically combine the explanation component with the embedding-based ranking part for the final prediction. Therefore, ECF is a truly coherent and self-explainable model with readable taste clusters.


\subsection{Model Analysis}


\subsubsection{\textbf{Model Size}} 
We analysis the size of ECF from both training and inference perspectives. During the training, the model parameters of single ECF consist of (1) ID embeddings of users and items $\{\Mat{U},\Mat{V} | \Mat{U}\in \Space{R}^{M\times d},\Mat{V}\in\Space{R}^{N\times d} \}$, which are also used by all embedding-based methods; and (2) ID embedding of taste clusters $\{\Mat{H}| \Mat{H}\in\Space{R}^{Z\times d} \}$. We utilize 9 different  ECF model for training, so that the overall parameters are 9 times of the single model parameters. During the inference, different from other embeddings-based methods, ECF only need the sparse affiliations between users/items and clusters for prediction, and the parameters are $9 (K\times N +F\times M)$, which is similar or even less than the typical embedding-based methods (\ie MF need $d (N+M)$ parameters) when $K, F \ll d$.


\subsubsection{\textbf{Time Complexity}}
Time cost of ECF mainly comes from the taste clusters learning. For collaborative similarity learning of taste clusters, the computational complexity of calculating the affiliations relationship is $O(ZN(d+ |\Mat{Y}|))$, where $Z$, $N$, $|\Mat{Y}|$ and $d$ denote the number of taste clusters, items, interactions, and the embedding size. For tag similarity learning, the computational complexity of tag distribution is $O(ZN|\bar{t}|)$, where $|\bar{t}|$ is the average number of tags that items have. As for independence modeling, the cost of mutual information is $O(dZ^2)$. Besides, computing the auxiliary collaborative signals would cost $O(MNd)$. Thus, the time complexity of the whole training epoch is $O(ZN(d+|\Mat{Y}|+M)+dZ^2)$. Under the same experimental settings
(i.e., same embeddings size and same number of tags), ECF has comparable complexity to EFM and AMCF, two representative explainable methods.


